Reachability-Preserving Bellman Operator for the Discounted Reach-Cost Value Function: Uniting Hamilton-Jacobi Reachability and Reinforcement Learning

Hamilton-Jacobi (HJ) reachability provides rigorous safety and reachability guarantees for continuous-time dynamical systems, but its numerical solution suffers from the curse of dimensionality. Deep reinforcement learning (DRL), by contrast, offers scalable sample-based methods. However, RL is typically built around additive cumulative rewards; whereas, reachability objectives are inherently non-additive. This mismatch makes a direct bridge between HJ reachability and RL nontrivial. Recent discounted formulations have either introduced contraction by altering the original reachability semantics, or preserved exact semantics on the HJ side without a corresponding Bellman fixed-point characterization. In this paper, we close this gap by building on a semantics-preserving discounted reach-based value function and deriving a non-additive Bellman operator whose unique fixed point exactly matches the value function in the HJ formulation. We prove that discounting makes this operator contractive, yielding existence, uniqueness, and convergence of value iteration. Furthermore, we establish the equivalence between the HJ and Bellman characterizations, and show that RL can be interpreted as a sample-based approximation scheme for the same fixed-point equation. This yields a principled and semantically exact connection between HJ reachability and RL, enabling learning-based methods to approximate reachability value functions while preserving their safety-critical meaning. As a result, the proposed framework opens the door to scalable, data-driven computation of reachable sets and safety certificates in high-dimensional systems. Numerical experiments demonstrate close agreement with HJ solutions, confirm preservation of reachability semantics via alignment of zero level sets, and support the interpretation of reinforcement learning as a sample-based solver of the proposed Bellman operator.

==> content/algorithms/fvi-finite.tex <==
\begin{algorithm}[t]
\caption{Finite-Horizon Fitted Value Iteration (Backward Time-Marching)}
\label{alg:fvi_finite}
\begin{algorithmic}[1]

\Require value function $\Psi_\theta^{(k)}$, reach cost $g$, control set $\mathcal{U}_d$, dynamics model, optimizer $\mathcal{O}$, sampling distribution $\rho$, batch size $B$, rollout horizon $M$, time step $\Delta t$, discount $(\lambda, \sigma)$, horizon $\tau^*$

\State $N \gets \tau^* / \sigma$

\vspace{0.5em}
\Statex \textbf{Initialization}

\State $\Psi_\theta^{(0)}(x) \gets g(x)$

\vspace{0.5em}
\Statex \textbf{Backward Time-Marching}

\For{$k = 0$ to $N-1$}

\State Initialize parameters $\theta$, $\bar{\theta} \gets \theta$

\For{$n = 1$ to $N_{\text{train}}$}

    \State Sample $\{x_i\}_{i=1}^{B} \sim \rho$

    \For{each $x_i$}
        \For{each $u \in \mathcal{U}_d$}

            \State Roll out trajectory $\{x_j^u\}_{j=0}^{M}$ from $x_i$
            
            \State $J_{\text{stop}}(u) \gets \min_{j=0,\dots,M} e^{-\lambda j \Delta t} g(x_j^u)$
            
            \State $J_{\text{cont}}(u) \gets e^{-\lambda \sigma} \Psi_{\bar{\theta}}^{(k)}(x_M^u)$
            
            \State $J(u) \gets \min(J_{\text{stop}}(u), J_{\text{cont}}(u))$

        \EndFor

        \State $y_i \gets \min_{u \in \mathcal{U}_d} J(u)$

    \EndFor

    \State $\theta \gets \theta - \mathcal{O} \nabla_\theta \frac{1}{B} \sum_i (\Psi_\theta^{(k+1)}(x_i) - y_i)^2$

    \State $\bar{\theta} \gets \tau \theta + (1 - \tau)\bar{\theta}$

\EndFor

\State $\Psi_\theta^{(k+1)} \gets \Psi_\theta$

\EndFor

\State \Return $\Psi_\theta^{(N)} \approx W(\tau^*, x)$

\end{algorithmic}
\end{algorithm}


==> content/algorithms/fvi-original.tex <==
\begin{algorithm}[t]
\caption{Fitted Value Iteration with Reachability Bellman Operator}
\label{alg:fvi_combined}
\begin{algorithmic}[1]

\Require value function $\Psi_\theta$ structure, reach cost $g$, control set $\mathcal{U}_d$, dynamics model, optimizer $\mathcal{O}$, sampling distribution $\rho$, batch size $B$, Bellman step $\sigma$, rollout horizon $H$, timestep $\Delta t$, discount rate $\lambda$, pre-training steps $N_{\text{pre}}$, convergence threshold $\epsilon$ %training steps $N_{\text{train}}$ , target update rate $\tau$

\State Initialize parameters $\theta$ %, $\bar{\theta} \gets \theta$

\vspace{0.5em}
\Statex \textbf{Pretraining on reach cost}

\For{$k = 1$ to $N_{\text{pre}}$}
    \State Sample $\{x_i\}_{i=1}^{B} \sim \rho$
    \State $y_i \gets g(x_i)$
    \State $\mathcal{L}_{\text{pre}}(\theta) \leftarrow \frac{1}{B} \sum_{i=1}^{B} \left( \Psi_\theta(x_i) - y_i \right)^2$
    \State $\theta \gets \mathcal{O}(\theta, \mathcal{L}_{\text{pre}}(\theta))$
\EndFor

\vspace{0.5em}
\Statex \textbf{Fitted value iteration}

% \For{$k = 1$ to $N_{\text{train}}$}
\While{$\frac{1}{B} \sum_{i=1}^{B} \left( \Psi_\theta(x_i) - \widehat{\mathcal{T}}^{\infty}_{\sigma,\lambda}(\Psi_\theta)(x_i) \right)^2 > \epsilon$}
% \While{error less than threshold}

    \State Sample $\{x_i\}_{i=1}^{B} \sim \rho$

    \For{each $x_i$}
        \For{each $u \in \mathcal{U}_d$}
            \State Roll out trajectory $\{x_j^u\}_{j=0}^{H}$ using dynamics
            \State $J_{\text{stop}}(u) \gets \min_{j=0,\dots,H} e^{-\lambda j \Delta t} g(x_j^u)$
            \State $J_{\text{cont}}(u) \gets e^{-\lambda \sigma} \Psi_{\theta}(x_H^u)$
            \State $J(u) \gets \min(J_{\text{stop}}(u), J_{\text{cont}}(u))$
        \EndFor
        \State $y_i \gets \min_{u \in \mathcal{U}} J(u)$
    \EndFor

    \State Compute the loss $\mathcal{L}(\theta)$ according to \cref{eq:loss_theta}

    \State $\theta \gets \mathcal{O}(\theta, \mathcal{L}(\theta))$

    % \State $\bar{\theta} \gets \tau \theta + (1 - \tau)\bar{\theta}$

% \EndFor
\EndWhile

\State \Return $\Psi_\theta$

\end{algorithmic}
\end{algorithm}

==> content/algorithms/fvi.tex <==
\begin{algorithm}
\caption{Finite-Horizon FVI with Reachability Bellman Operator}
\label{alg:fvi-finite}
\begin{algorithmic}[1]
\Require value function $\Psi_\theta(\tau, \cdot)$ structure, reach cost $g$, control set 
$\mathcal{U}_d$, dynamics model, optimizer $\mathcal{O}$, sampling distribution $\rho$ over 
$[0,T] \times \mathbb{R}^n$, batch size $B$, Bellman step $\sigma$, timestep $\Delta t$, 
discount rate $\lambda$, pre-training steps $N_\text{pre}$, convergence threshold $\epsilon$

\State Initialize parameters $\theta$

\Statex \textit{Pretraining on reach cost (enforces boundary condition $\Psi_\theta(0, x) = g(x)$)}
\For{$k = 1$ to $N_\text{pre}$}
    \State Sample $\{x_i\}_{i=1}^B \sim \rho(\cdot \mid \tau = 0)$
    \State $y_i \leftarrow g(x_i)$
    \State $\mathcal{L}_\text{pre}(\theta) \leftarrow \frac{1}{B} \sum_{i=1}^B \left(\Psi_\theta(0, x_i) - y_i\right)^2$
    \State $\theta \leftarrow \mathcal{O}(\theta, \mathcal{L}_\text{pre}(\theta))$
\EndFor

\Statex \textit{Fitted value iteration}
\While{$\frac{1}{B}\sum_{i=1}^B \left(\Psi_\theta(\tau_i, x_i) - \hat{T}_{\sigma,\lambda}(\Psi_\theta)(\tau_i, x_i)\right)^2 > \epsilon$}
    \State Sample $\{(\tau_i, x_i)\}_{i=1}^B \sim \rho$
    \For{each $(\tau_i, x_i)$}
        \State Set $h_i \leftarrow \min\{\tau_i, \sigma\}$, $H_i \leftarrow h_i / \Delta t$
        \For{each $u \in \mathcal{U}_d$}
            \State Roll out trajectory $\{x^u_j\}_{j=0}^{H_i}$ using dynamics
            \State $J_\text{stop}(u) \leftarrow \min_{j=0,\ldots,H_i} e^{-\lambda j \Delta t} g(x^u_j)$
            \State $J_\text{cont}(u) \leftarrow e^{-\lambda h_i} \Psi_\theta(\tau_i - h_i,\, x^u_{H_i})$
            \State $J(u) \leftarrow \min(J_\text{stop}(u),\, J_\text{cont}(u))$
        \EndFor
        \State $y_i \leftarrow \min_{u \in \mathcal{U}_d} J(u)$
    \EndFor
    \State $\mathcal{L}(\theta) \leftarrow \frac{1}{B} \sum_{i=1}^B \left(\Psi_\theta(\tau_i, x_i) - y_i\right)^2$
    \State $\theta \leftarrow \mathcal{O}(\theta, \mathcal{L}(\theta))$
\EndWhile
\State \Return $\Psi_\theta$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Infinite-Horizon FVI with Reachability Bellman Operator}
\label{alg:fvi-infinite}
\begin{algorithmic}[1]
\Require value function $\Psi_\theta$ structure, reach cost $g$, control set $\mathcal{U}_d$, 
dynamics model, optimizer $\mathcal{O}$, sampling distribution $\rho$ over $\mathbb{R}^n$, 
batch size $B$, Bellman step $\sigma$, timestep $\Delta t$, discount rate $\lambda$, 
convergence threshold $\epsilon$

\State Initialize parameters $\theta$

\Statex \textit{Fitted value iteration}
\While{$\frac{1}{B}\sum_{i=1}^B \left(\Psi_\theta(x_i) - \hat{T}^\infty_{\sigma,\lambda}(\Psi_\theta)(x_i)\right)^2 > \epsilon$}
    \State Sample $\{x_i\}_{i=1}^B \sim \rho$
    \For{each $x_i$}
        \For{each $u \in \mathcal{U}_d$}
            \State Roll out trajectory $\{x^u_j\}_{j=0}^{H}$ using dynamics, where $H = \sigma/\Delta t$
            \State $J_\text{stop}(u) \leftarrow \min_{j=0,\ldots,H} e^{-\lambda j \Delta t} g(x^u_j)$
            \State $J_\text{cont}(u) \leftarrow e^{-\lambda\sigma} \Psi_\theta(x^u_H)$
            \State $J(u) \leftarrow \min(J_\text{stop}(u),\, J_\text{cont}(u))$
        \EndFor
        \State $y_i \leftarrow \min_{u \in \mathcal{U}_d} J(u)$
    \EndFor
    \State $\mathcal{L}(\theta) \leftarrow \frac{1}{B} \sum_{i=1}^B \left(\Psi_\theta(x_i) - y_i\right)^2$
    \State $\theta \leftarrow \mathcal{O}(\theta, \mathcal{L}(\theta))$
\EndWhile
\State \Return $\Psi_\theta$
\end{algorithmic}
\end{algorithm}

\begin{boxedremark}[Relationship between \cref{alg:fvi-finite} and \cref{alg:fvi-infinite}]
\cref{alg:fvi-infinite} specializes \cref{alg:fvi-finite} to the stationary setting in three ways: 
(i) pretraining is omitted since $\mathcal{V}^\infty$ imposes no boundary condition 
(see \cref{def:B-infinity}), and Banach's theorem guarantees convergence from 
any bounded initialization; (ii) rollouts always run the full $H = \sigma/\Delta t$ steps 
since there is no remaining time constraint, whereas in Algorithm~1 rollouts are truncated 
to $H_i = h_i/\Delta t$ steps when $\tau_i < \sigma$; and (iii) the network $\Psi_\theta$ 
takes only $x$ as input rather than $(\tau, x)$, reflecting the stationarity of $W^\infty$.
\end{boxedremark}
